An IoT application development using IoTSuite

Application development in the Internet of Things (IoT) is challenging because it involves dealing with issues that attribute to different life-cycle phases. First, the application logic has to be analyzed and then separated into a set of distributed tasks for an underlying network. Then, the tasks have to be implemented for the specific hardware. Moreover, we take different IoT applications and present development of these applications using IoTSuite. In this paper, we introduce a design and implementation of ToolSuite, a suite of tools, for reducing burden of each stage of IoT application development process. We take different class of IoT applications, largely found in the IoT literature, and demonstrate these IoT application development using IoTSuite. These applications have been tested on several IoT technologies such as Android, Raspberry PI, Arduino, and JavaSE-enabled devices, Messaging protocols such as MQTT, CoAP, WebSocket, Server technologies such as Node.js, Relational database such as MySQL, and Microsoft Azure Cloud services.

==> Arxiv version of ToolSuite Journal Paper/introduction.tex <==
\section{Introduction}

Recent technological advances in computer and communication technology 
have been fueling a tremendous growth in a number of smart
objects (or \emph{things})~\cite{vasseur2010interconnecting}.
In the Internet of Things\footnote{\url{http://www.grifs-project.eu/data/File/CASAGRAS\%20FinalReport\%20(2).pdf}}, 
these ``things'' acquire intelligence, thanks to the fact that they access information 
that has been aggregated by other things.  For example, a building interacts 
with its residents and surrounding buildings in case of fire for safety and security of residents, 
offices adjust themselves automatically accordingly to user preferences while minimizing energy consumption, 
or traffic signals control in-flow of vehicles according to the current highway status~\cite{de2009internet,IoTsurvey}. 
It is the goal of our work to enable the development of such applications. 
In the following, we discuss one of such applications. 

\subsection{Challenges and contributions}
Application development in the IoT is challenging because stakeholders\footnote{we will use the term stakeholders as
used in software engineering to mean people, who are involved in the application development.
Examples of stakeholders defined in~\cite{softwareArchtaylor2010}  are software designer, developer, domain
expert, technologist, etc.} have to address issues that are attributed 
to different life cycles phases, including development, deployment, and maintenance~\cite{bischoff2007life}. 
At the \textbf{\emph{development phase}}, the application logic has to be analyzed and separated into a set of distributed 
tasks for the underlying network consisting of a large number of heterogeneous entities. 
Then, the tasks have to be  implemented for  the specific platform of a device. At the \textbf{\emph{deployment phase}}, the application logic has to be deployed onto a large number of devices. Manual effort in above two phases for hundreds to thousands of heterogeneous devices is a time-consuming and error-prone process.   

An important challenge that needs to be addressed in the IoT is to enable the rapid development 
of applications with minimal effort by stakeholders involved in the process~\cite{patel:hal-00788366, DBLP:journals/corr/PatelLB16}.
In our previous publications~\cite{patelhalscube,  Chauhan:2016:DFP:2897035.2897039, patel-icse14}, we have provided a complete tour of our
IoT application development process, summarized in Section~\ref{sec:ourapproach}. 
This paper goes beyond it. In particular, it describes implementation technologies, tools, language used and their 
rationales of choosing them~\cite{patel-comnet-iot15, 7460669, 7467275}. Although various efforts exist in literature for making IoT 
application development easier, very few of them are publicly available for stakeholders to 
choose from. Given the usefulness of open source, our aim is to provide an opportunity 
to community for the creation of novel software engineering tools and the conduction 
of novel research for IoT application development.  

The main contribution of this paper is an implementation of ToolSuite, a suite of tools,
for reducing burden at different phases for IoT application 
development~(detail in Section~\ref{sec:components}). Moreover, we take 
different class of IoT applications~\cite{appdevIoTpatel2011} and describe
an application development process using IoTSuite. 

\textbf{Outline.} The remainder of this paper is organized as follows: Section \ref{sec:ourapproach} presents the development framework that includes the proposed modeling languages and automation techniques. Section \ref{sec:components} presents the implementation of the development framework and describes implementation technologies, tools, and languages used. Section \ref{sec:appdev} describes step by step IoT application development process using IoTSuite. It also focus on different class of application to demonstrate application development using IoTSuite. Finally, in Section
~\ref{sec:conclusion}, we conclude this article and briefly mention some of future directions. 

==> Arxiv version of ToolSuite Journal Paper/ourapproach.tex <==
\section{IoT application development process}\label{sec:ourapproach}

This section presents our development framework that separates IoT application development into different concerns, namely \emph{domain}, \emph{platform}, \emph{functional}, and \emph{deployment}. It integrates a set of high-level modeling languages to specify such concerns.  These languages are supported by automation techniques at various phases of application development process. Stakeholders carry out the following steps in order to develop an IoT using our approach:

\begin{figure*}[!ht]
\centering
\includegraphics[width=0.7\textwidth]{figure-pdf-files/developmentframework.pdf}
\caption{IoT application development: the overall process}
\label{fig:devcycle}
\end{figure*}

\subsection{Domain Concern} 

This concern is related to concepts that are specific to a domain (e.g., building automation, transport) of an IoT. The stakeholders task regarding such 
concern consists of the following step:

\fakeparagraph{\em Specifying and compiling domain specification} 
The domain expert specifies a domain specification using the Domain Language~(DL) 
(Step~\circled{1} in Figure~\ref{fig:devcycle}). The domain specification includes specification of resources, which are responsible for interacting with Entities of Interest~(EoI). This includes \emph{tags}~(identify EoI), \emph{sensors}~(sense EoI), \emph{actuators}~(affect EoI), and \emph{storage}~(store information about EoI). In the domain specification, resources  are specified in a high-level manner to abstract low-level details from the domain expert.
%~(detail in Section~\ref{sec:specdomain}).
\subsection{Functional Concern}
This concern is related to concepts that are specific to functionality of an IoT application. An example of a functionality is to open a window when an average temperature value of a room is greater than $30^{\circ} C$. The stakeholders task regarding such 
concern consists of the following steps: 

\fakeparagraph{\em Specifying application architecture} 
Referring the domain specification, the software designer specifies an application architecture using the Architecture Language~(AL)-(Step \circled{2} in Figure~\ref{fig:devcycle}). It consists of specification of computational 
services and interaction among them. A computational service is fueled by sensors and storage defined in the domain specification. They process inputs data and take appropriate decisions by triggering actuators defined in the domain specification. The application architecture  consists of \textit{common} operations and \textit{custom} components that are specific to the application logic.

\fakeparagraph{\em Implementing application logic} 
The compilation of an architecture specification generates an architecture framework~(Step~\circled{3} 
in Figure~\ref{fig:devcycle}).  The architecture framework contains abstract classes, 
corresponding to  each  computational service, that hide interaction details with other 
software components  and allow the application developer to focus only  on application logic. 
The application developer implements only abstract methods of generated abstract classes, described in our work~\cite[p.~73]{Patel201562}.
We have integrated a framework for common operations. This further reduces the development effort  for commonly found operations in IoT application and provides re-usability. 

\subsection{Platform Concern}
This concern specifies the concepts that fall into computer 
programs that act as a translator between a hardware device and an application. 
The stakeholders task regarding such concern consists of the following steps:
		
\fakeparagraph{\em Generating device drivers}
The compilation of domain specification generates a domain framework~(Step~\circled{4} in Figure~\ref{fig:devcycle}). 
It contains {\em concrete classes} corresponding to concepts defined in the domain specification. The concrete classes contain concrete
methods to interact with other software components and platform-specific device drivers,
described in our work~\cite[p.~75]{Patel201562}. We have integrated existing open-source sensing framework\footnote{\url{http://www.funf.org/}} 
for Android devices. Moreover, we have implemented sensing and actuating framework
for Raspberry Pi and storage framework for MongoDB, MySQL, and Microsoft AzureDB. So, the device developers do not have to implement platform-specific sensor, actuator, and storage code.

\fakeparagraph{\em Specifying user interactions}
To define user interactions, we present a set of {\em abstract interactors}, similar to work~\cite{Balland-2013}, that denotes information exchange between an application and a user. The software designer specifies them using User Interaction Language~(UIL)~(Step~\circled{5} in Figure~\ref{fig:devcycle}). 


\fakeparagraph{\em Implementing user-interface code}
Leveraging the user interaction specification, the development framework generates a User Interface~(UI) framework~(step~\circled{6} in Figure~\ref{fig:devcycle}). The UI framework contains a set of {\em interfaces} and {\em concrete classes} corresponding to resources defined in the user interaction specification.  The concrete classes contain concrete methods for interacting with other software components. 
The user interface designer implements {\em interfaces}. These interfaces implement code that connects appropriate UI elements to concrete methods. 
For instance, a user initiates a command to heater by pressing UI element such as \texttt{button} that invokes a \texttt{sendCommandToHeater()} concrete method.
 
\subsection{Deployment Concern}

This concern is related to deployment-specific concepts that describe the
information about a device and its properties placed in the target deployment. 
It consists of the following steps:

\fakeparagraph{\em Specifying target deployment} 
Referring the domain specification, the network manager describes a deployment specification using the Deployment Language~(DL)~(Step~\circled{7} in Figure~\ref{fig:devcycle}). The deployment specification 
includes the details of each device as well as abstract interactors specified in the
user interaction specification.

\fakeparagraph{Mapping} The mapper takes a set of devices defined in the deployment specification and  a set of computation components defined in the architecture specification(Step-~\circled{8} in Figure~\ref{fig:devcycle}). It maps computational service to a device.  The current version of mapper algorithm~\cite{Patel201562} selects devices randomly and allocates computational services to the selected devices.

\subsection{Linking}
The linker combines the code generated by various stag-es and creates packages that can be deployed on devices~(St-ep~\circled{9} in Figure~\ref{fig:devcycle}).  This stage supports the application deployment phase by producing device-specific code to result in a distributed software system collaboratively hosted by individual devices, thus providing automation at the deployment phase.

The final output of linker is composed of three parts: (1) a \emph{runtime-system} runs on each individual device and provides a support for executing distributed tasks, (2) a \emph{device-specific code} generated by the linker module, and (3) a \emph{wrapper} separates generated code from the linker module and underlying runtime system by implementing interfaces. 

==> introduction.tex <==
\section{Introduction}

Recent technological advances in computer and communication technology 
have been fueling a tremendous growth in a number of smart
objects (or \emph{things})~\cite{vasseur2010interconnecting}.
In the Internet of Things\footnote{\url{http://www.grifs-project.eu/data/File/CASAGRAS\%20FinalReport\%20(2).pdf}}, 
these ``things'' acquire intelligence, thanks to the fact that they access information 
that has been aggregated by other things.  For example, a building interacts 
with its residents and surrounding buildings in case of fire for safety and security of residents, 
offices adjust themselves automatically accordingly to user preferences while minimizing energy consumption, 
or traffic signals control in-flow of vehicles according to the current highway status~\cite{de2009internet,IoTsurvey}. 
It is the goal of our work to enable the development of such applications. 
In the following, we discuss one of such applications. 

\subsection{Challenges and contributions}
Application development in the IoT is challenging because stakeholders\footnote{we will use the term stakeholders as
used in software engineering to mean people, who are involved in the application development.
Examples of stakeholders defined in~\cite{softwareArchtaylor2010}  are software designer, developer, domain
expert, technologist, etc.} have to address issues that are attributed 
to different life cycles phases, including development, deployment, and maintenance~\cite{bischoff2007life}. 
At the \textbf{\emph{development phase}}, the application logic has to be analyzed and separated into a set of distributed 
tasks for the underlying network consisting of a large number of heterogeneous entities. 
Then, the tasks have to be  implemented for  the specific platform of a device. At the \textbf{\emph{deployment phase}}, the application logic has to be deployed onto a large number of devices. Manual effort in above two phases for hundreds to thousands of heterogeneous devices is a time-consuming and error-prone process.   

An important challenge that needs to be addressed in the IoT is to enable the rapid development 
of applications with minimal effort by stakeholders involved in the process~\cite{patel:hal-00788366, DBLP:journals/corr/PatelLB16}.
In our previous publications~\cite{patelhalscube,  Chauhan:2016:DFP:2897035.2897039, patel-icse14}, we have provided a complete tour of our
IoT application development process, summarized in Section~\ref{sec:ourapproach}. 
This paper goes beyond it. In particular, it describes implementation technologies, tools, language used and their 
rationales of choosing them~\cite{patel-comnet-iot15, 7460669, 7467275}. Although various efforts exist in literature for making IoT 
application development easier, very few of them are publicly available for stakeholders to 
choose from. Given the usefulness of open source, our aim is to provide an opportunity 
to community for the creation of novel software engineering tools and the conduction 
of novel research for IoT application development.  

The main contribution of this paper is an implementation of ToolSuite, a suite of tools,
for reducing burden at different phases for IoT application 
development~(detail in Section~\ref{sec:components}). Moreover, we take 
different class of IoT applications~\cite{appdevIoTpatel2011} and describe
an application development process using IoTSuite. 

\textbf{Outline.} The remainder of this paper is organized as follows: Section \ref{sec:ourapproach} presents the development framework that includes the proposed modeling languages and automation techniques. Section \ref{sec:components} presents the implementation of the development framework and describes implementation technologies, tools, and languages used. Section \ref{sec:appdev} describes step by step IoT application development process using IoTSuite. It also focus on different class of application to demonstrate application development using IoTSuite. Finally, in Section
~\ref{sec:conclusion}, we conclude this article and briefly mention some of future directions. 

==> ourapproach.tex <==
\section{IoT application development process}\label{sec:ourapproach}

This section presents our development framework that separates IoT application development into different concerns, namely \emph{domain}, \emph{platform}, \emph{functional}, and \emph{deployment}. It integrates a set of high-level modeling languages to specify such concerns.  These languages are supported by automation techniques at various phases of application development process. Stakeholders carry out the following steps in order to develop an IoT using our approach:

\begin{figure*}[!ht]
\centering
\includegraphics[width=0.7\textwidth]{figure-pdf-files/developmentframework.pdf}
\caption{IoT application development: the overall process}
\label{fig:devcycle}
\end{figure*}

\subsection{Domain Concern} 

This concern is related to concepts that are specific to a domain (e.g., building automation, transport) of an IoT. The stakeholders task regarding such 
concern consists of the following step:

\fakeparagraph{\em Specifying and compiling domain specification} 
The domain expert specifies a domain specification using the Domain Language~(DL) 
(Step~\circled{1} in Figure~\ref{fig:devcycle}). The domain specification includes specification of resources, which are responsible for interacting with Entities of Interest~(EoI). This includes \emph{tags}~(identify EoI), \emph{sensors}~(sense EoI), \emph{actuators}~(affect EoI), and \emph{storage}~(store information about EoI). In the domain specification, resources  are specified in a high-level manner to abstract low-level details from the domain expert.
%~(detail in Section~\ref{sec:specdomain}).
\subsection{Functional Concern}
This concern is related to concepts that are specific to functionality of an IoT application. An example of a functionality is to open a window when an average temperature value of a room is greater than $30^{\circ} C$. The stakeholders task regarding such 
concern consists of the following steps: 

\fakeparagraph{\em Specifying application architecture} 
Referring the domain specification, the software designer specifies an application architecture using the Architecture Language~(AL)-(Step \circled{2} in Figure~\ref{fig:devcycle}). It consists of specification of computational 
services and interaction among them. A computational service is fueled by sensors and storage defined in the domain specification. They process inputs data and take appropriate decisions by triggering actuators defined in the domain specification. The application architecture  consists of \textit{common} operations and \textit{custom} components that are specific to the application logic.

\fakeparagraph{\em Implementing application logic} 
The compilation of an architecture specification generates an architecture framework~(Step~\circled{3} 
in Figure~\ref{fig:devcycle}).  The architecture framework contains abstract classes, 
corresponding to  each  computational service, that hide interaction details with other 
software components  and allow the application developer to focus only  on application logic. 
The application developer implements only abstract methods of generated abstract classes, described in our work~\cite[p.~73]{Patel201562}.
We have integrated a framework for common operations. This further reduces the development effort  for commonly found operations in IoT application and provides re-usability. 

\subsection{Platform Concern}
This concern specifies the concepts that fall into computer 
programs that act as a translator between a hardware device and an application. 
The stakeholders task regarding such concern consists of the following steps:
		
\fakeparagraph{\em Generating device drivers}
The compilation of domain specification generates a domain framework~(Step~\circled{4} in Figure~\ref{fig:devcycle}). 
It contains {\em concrete classes} corresponding to concepts defined in the domain specification. The concrete classes contain concrete
methods to interact with other software components and platform-specific device drivers,
described in our work~\cite[p.~75]{Patel201562}. We have integrated existing open-source sensing framework\footnote{\url{http://www.funf.org/}} 
for Android devices. Moreover, we have implemented sensing and actuating framework
for Raspberry Pi and storage framework for MongoDB, MySQL, and Microsoft AzureDB. So, the device developers do not have to implement platform-specific sensor, actuator, and storage code.

\fakeparagraph{\em Specifying user interactions}
To define user interactions, we present a set of {\em abstract interactors}, similar to work~\cite{Balland-2013}, that denotes information exchange between an application and a user. The software designer specifies them using User Interaction Language~(UIL)~(Step~\circled{5} in Figure~\ref{fig:devcycle}). 


\fakeparagraph{\em Implementing user-interface code}
Leveraging the user interaction specification, the development framework generates a User Interface~(UI) framework~(step~\circled{6} in Figure~\ref{fig:devcycle}). The UI framework contains a set of {\em interfaces} and {\em concrete classes} corresponding to resources defined in the user interaction specification.  The concrete classes contain concrete methods for interacting with other software components. 
The user interface designer implements {\em interfaces}. These interfaces implement code that connects appropriate UI elements to concrete methods. 
For instance, a user initiates a command to heater by pressing UI element such as \texttt{button} that invokes a \texttt{sendCommandToHeater()} concrete method.
 
\subsection{Deployment Concern}

This concern is related to deployment-specific concepts that describe the
information about a device and its properties placed in the target deployment. 
It consists of the following steps:

\fakeparagraph{\em Specifying target deployment} 
Referring the domain specification, the network manager describes a deployment specification using the Deployment Language~(DL)~(Step~\circled{7} in Figure~\ref{fig:devcycle}). The deployment specification 
includes the details of each device as well as abstract interactors specified in the
user interaction specification.

\fakeparagraph{Mapping} The mapper takes a set of devices defined in the deployment specification and  a set of computation components defined in the architecture specification(Step-~\circled{8} in Figure~\ref{fig:devcycle}). It maps computational service to a device.  The current version of mapper algorithm~\cite{Patel201562} selects devices randomly and allocates computational services to the selected devices.

\subsection{Linking}
The linker combines the code generated by various stag-es and creates packages that can be deployed on devices~(St-ep~\circled{9} in Figure~\ref{fig:devcycle}).  This stage supports the application deployment phase by producing device-specific code to result in a distributed software system collaboratively hosted by individual devices, thus providing automation at the deployment phase.

The final output of linker is composed of three parts: (1) a \emph{runtime-system} runs on each individual device and provides a support for executing distributed tasks, (2) a \emph{device-specific code} generated by the linker module, and (3) a \emph{wrapper} separates generated code from the linker module and underlying runtime system by implementing interfaces. 
